Dynamic Network Model from Partial Observations

Can evolving networks be inferred and modeled without directly observing their nodes and edges? In many applications, the edges of a dynamic network might not be observed, but one can observe the dynamics of stochastic cascading processes (e.g., information diffusion, virus propagation) occurring over the unobserved network. While there have been efforts to infer networks based on such data, providing a generative probabilistic model that is able to identify the underlying time-varying network remains an open question. Here we consider the problem of inferring generative dynamic network models based on network cascade diffusion data. We propose a novel framework for providing a non-parametric dynamic network model--based on a mixture of coupled hierarchical Dirichlet processes-- based on data capturing cascade node infection times. Our approach allows us to infer the evolving community structure in networks and to obtain an explicit predictive distribution over the edges of the underlying network--including those that were not involved in transmission of any cascade, or are likely to appear in the future. We show the effectiveness of our approach using extensive experiments on synthetic as well as real-world networks.

==> sections/1_Introduction_copy.tex <==
% !TEX root=../nips_2018.tex

\section{Introduction}
\label{sec:Introduction}
Networks of interconnected entities are widely used to model pairwise relations between nodes or entities in many important problems in sociology, finance, computer science, and  operations research \cite{namaki2011network, myers2010convexity, ahmed2009recovering}. In many real-world problems, however, the underlying network structure is not known, and we can only observe the spread of contagions (e.g. information propagation, adoption of new products/innovations, spread of infections, etc.) over the network. The observations are often in the form of the time when different nodes adopt a contagion. A fundamental problem, therefore, is to infer the underlying network structure from these observations.

A contagion appears at some node of a network and
then spreads like an epidemic from node to node over the edges of

%We don't need to have a model of diffusion processes/ models of edge transmission likelihood
In recent years, there has been a large body of research on inferring
the structure of networks over which various types of contagions
spread \cite{myers2010convexity, gomez2011uncovering, gomez2010inferring, rodriguez2012submodular}. However, these efforts are mostly limited to inferring the set of most likely edges between infected nodes (assuming a fixed transmission model), %by formulating the problem as a submodular or convex optimization. There has been recent efforts on using
or more recently, predicting the set of nodes that can possibly be infected next \cite{bourigault2016representation, wang2017topological}. To the best of our knowledge, none of the existing methods are able to provide a generative probabilistic model for the underlying network, and infer the latent network structure from partial observation.
 
Often times, networks over which information propagates are not static. Nodes or edges appear or disappear, and the underlying community structure changes over time. Therefore, we are often interested in modeling, and understanding the structure of dynamic networks with an unbounded number of nodes and edges. %, or on the rate of appearance and disappearance of nodes and edges in the network. Such models allow us to capture the evolution of the underlying network structure and predict its future dynamics. 
%
%Some approaches infer the underlying diffusion networks as a sequence of binary edges \cite{gomez2010inferring, snowsill2011refining}, while others are also able to infer the transmission probabilities \cite{gomez2011uncovering, myers2010convexity}. However, they mostly rely on the assumption that transmission probabilities are generated from a known probability distribution.  Furthermore, the existing methods only focus on inferring the edges (and their transmission probabilities), and are not able to provide a  probabilistic model to captures the latent structural properties of the network and enables us to predict its future interactions and structural properties.
%for the underlying network structure. 
%Having a model from the underlying network structure is important as it
%Such leads to new insights about the network structural properties, e.g. community structures, degree distribution, etc. In addition, it 
%Such models may lead to new insights about the structural properties of networks and allow to predict future interactions.
%
Non-parametric models are specially useful when we don't have any prior knowledge or assumption about the shape or size of the network.
There has been a body of work on designing non-parametric network models from full observations \cite{holland1983stochastic, snijders1997estimation, williamson2016nonparametric, cai2016edge}. 
They mostly rely on the assumption of vertex exchangeability, in which the distribution of a graph is invariant to the order of its vertices \cite{holland1983stochastic, snijders1997estimation}. 
While vertex-exchangeable models are well-suited to community detection, they are less appropriate for the task of predicting unseen interactions.  Moreover, they are not appropriate for modeling sparse networks.
%One limitation of vertex-exchangeable models is that they generate either dense or empty graphs with probability one \cite{orbanz2015bayesian, wang1987stochastic}, which contradicts the sparse nature of many real-world networks. 
Very recently, an alternative notion of edge-exchangeability was introduced for graphs, in which the distribution of a graph is invariant to the order of its edges \cite{williamson2016nonparametric, cai2016edge}. Unlike the traditional vertex-exchangeable models, edge-exchangeable models can exhibit sparsity, and small-world behavior of real networks.
They allow both the latent dimensionality of the model and the number of nodes in the network to grow over time, and are suitable for predicting future interactions.

In this work, we propose a novel on-line dynamic network inference framework, \alg, for providing non-parametric edge-exchangeable network models from partial observations.
We build upon the non-parametric network model of \cite{williamson2016nonparametric} that places a mixture of Dirichlet processes over the outgoing and incoming edges in each community, and couples the network using a shared discrete base measure.
For each time interval, we process the corresponding diffusion data in an iterative manner. 
First, we find the most probable diffusion tree supported by each cascade. We then provide the edges of the trees as observations to an MCMC sampler and update our non-parametric model. 
In the next iteration, the updated transmission probabilities provided by the model are used to update the most probable diffusion trees. We continue the above iterative process until the model does not change considerably.
%
Extensive experiments on synthetic and real-world networks show that \alg is able to track changes in the structure of dynamic networks and provides accurate on-line estimates of the time-varying edge probabilities for different network topologies.
%In addition, \alg has a superior predictive performance having only a small set of cascades.
We also applied \alg to predict the set of most influential nodes of MemeTracker over 150 days, and showed that...

%and fall under the stochastic block model (SB) framework \cite{}. Here, the nodes are assumed to belong to subgroups called blocks or communities, and there exists a fixed, stationary network between these nodes.



we usually think of diffusion as a process that takes place on a network,
where the contagion propagates over the edges of the underlying network from node
to node like an epidemic.


 

==> sections/3_problem.tex <==
% !TEX root=../nips_2018.tex

\section{Preliminaries}
In this section, we first formally define the problem of dynamic network inference from partial observations. We then review the non-parametric edge-exchangeable network model of [8] that we will build upon in the rest of this paper. Finally, we give a brief overview of Bayesian inference for inferring latent model variables.

\subsection{Dynamic Network Inference Problem}\label{sec:problem}
Consider a hidden directed dynamic network where nodes and edges may appear or disappear over time. At each time step $t$, the network $G^t=(V^t, E^t)$ consists of a set of vertices $V^t$, and a set of edges $E^t$.
We assume that $V^1 \subseteq V^2 \cdots \subseteq V$. However, we consider a node as disappeared if it doesn't have any edges.
A set $C$ of $s$ contagions spread over edges of the network from infected to non-infected nodes. For each contagion $c \in C$, we observe a cascade $t^c := (t_1^c, \cdots, t_{|V|}^c)$, recording the times when each node got infected by the contagion $c$. If a node $u$ is not infected by the contagion $c$, we set $t_u^c=\infty$. 
For each cascade, we only observe the time $t^c_u$ when a node $u$ got infected, but not who infected the node.
%We assume that contagions are propagating through the network independently of each other.
%Our goal is to infer the underlying unknown latent structure of the dynamic network $G^t$ over which cascades propagated using partial observations, i.e. infection times. 
Our goal is to infer a model $\mathcal{M}^t$ to capture the latent structure of the dynamic network $G^t$ over which cascades propagated, using partial observations. 
Such a model, in particular, can provide us with the probabilities of the $M^t=|V^t|^2$ potential edges between all nodes $u,v\in V^t$.
%In particular, at any time step $t$, we want to infer the probability $p^t_{uv}$ of all possible $M^t=|V^t|^2$ edges between all $u,v\in V^t$, where $N^t=|V^t|$.

\subsection{Non-parametric Edge-exchangeable Network Model}
In order to have a flexible model that allows the network to grow over time, we adopt the Bayesian non-parametrics model of [8]. Here, the network is modeled as an exchangeable sequence of directed binary links. 
More specifically, each community in the network is modeled by a mixture of Dirichlet network distributions (MDND). For every community $k$, two Dirichlet distribution $A_k$, and $B_k$ are associated to the outlinks and inlinks in community $k$. To allow links between the communities associated with each mixture component, the network is coupled using a shared, discrete base measure $H$. The model $\mathcal{M}$ can be described as:
\begin{align}
\label{eq:mdnd}
%\begin{split}
D & \coloneqq (d_k, k \in \mathbb N) \sim \text{GEM}(\alpha) & c_{uv}&\sim D ~~~~~~~~~~~~~u,v \in V\\\nonumber
H & \coloneqq \sum_{i=1}^\infty h_i\delta_{\theta_i} \sim \text{DP}(\gamma,\Theta) & u &\sim A_{c_{uv}} \\\nonumber
A_k & \coloneqq \sum_{i=1}^\infty a_{k,i}\delta_{\theta_i} \sim \text{DP}(\tau, H) & v &\sim B_{c_{uv}}\\\nonumber
B_k & \coloneqq \sum_{i=1}^\infty b_{k,i}\delta_{\theta_i} \sim \text{DP}(\tau,H) & z_{ij} &= \sum_{u,v \in V}\mathbb{I}(u = i, v = j)
%\end{split}
\end{align}
where $\Theta$ is the measurable space, and $\text{GEM}(\alpha)$ is the stick-breaking distribution with parameter $\alpha$ that  controls the number of clusters. The concentration parameter $\tau$ controls the overlap between clusters, and $\gamma$ controls the total number of nodes in the network.
%For brevity, we show the above non-paramteric model with $\mathcal{M}(\theta)$, where $\theta$ is the infinite dimensional vector of parameters of the non-parametric model specified in (\ref{eq:mdnd}). 
%is the distribution over the size-biased atom sizes of a Dirichlet process with concentration parameter $\alpha$, and .
%To ensure the two distributions have the same support (meaning that any node can have both incoming and outgoing links), we couple these two distributions via a shared, discrete base measure $H$.

\subsection{Bayesian Inference}
Having specified the model in terms of the joint distribution in (\ref{eq:mdnd}), we need to estimate the posterior distribution of the latent variables in our network model conditioned on partial observations $X$:
\begin{equation}
p(\theta|X, \mathcal{M})=\frac{p(X|\theta, \mathcal{M})p(\theta|\mathcal{M})}{\int p(X,\theta|\mathcal{M}) d\theta} %p(\theta|\mathcal{M})
\end{equation}
Here $\theta$ is the infinite dimensional parameter vector of the non-parametric model specified in (\ref{eq:mdnd}). %we need to use approximate inference.
In Section \ref{sec:dynamic}, we show how we provide the diffusion data to a Gibbs sampler that iteratively samples from the conditional distribution $p(X|\theta, \mathcal{M})$, and approximate the posterior distribution $p(\theta|X, \mathcal{M})$. 









\section{\alg: Dynamic Network Inference from Partial Observations}\label{sec:dynamic}

In this section, %we first explain the dynamic network inference problem. 
we describe our algorithm, \alg, for inferring the latent strucutre of the underlying dynamic network from diffusion data. \alg works based on the following iterative idea: in each iteration we first find the most probable tree for each cascade. We then provide the set of edges associated with the most probable trees as observations to a Gibbs sampler that updates the posterior distribution of the latent variables of our non-parametric network model.


\subsection{Modeling Observations from Diffusion Data}
%In the first part, we
%Without any prior knowledge about the underlying network, we assume that 
%\bm{Without loss of generality, for any pair of infection times ($t_u^c$,  $t_v^c$) in cascade $c$, %the %pairwise transmission likelihood we model the likelihood of an edge $e_{uv}$ between infected nodes $u$ and $v$ as a exponentially decaying function of the difference between infection times, $\Delta^c_{u,v}=t^c_v-t^c_u$. I.e., for every $t_u < t_v \leq t$ we have:}
%initial probability of an edge $(u,v)$ between nodes $u$, and $v$ depends only on the time difference between the node hit times, $\Delta_{u,v}=t^c_v-t^c_u$. For simplicity, we model this dependence by an exponential function, i.e.,
%%%\begin{equation}
%f(e_{uv} |  t_u, t_v, \theta) \propto \sum_{c \in C} p(e_{uv}|\theta) ( 1 + e^{-(t_v^c-t_u^c)}),
%%%%%f^{t}_{c}(e_{uv}|t^c_u, t^c_v, \theta) = p^{t-1}(e_{uv}|\theta)
%(1+e^{-\Delta^c_{u,v}}). 
%f_c(t_v^c|t^c_u) %
%%%\end{equation}
%where $\alpha_{uv}$ is the pairwise transmission rate between nodes $u$ and $v$.
%Without any prior knowledge about the structure of the underlying network, we initialize $p^0(.) \propto \Delta^c_{u,v}=t^c_v-t^c_u$ for all the edges.
%In the end, our algorithm does not depend on the particular choice of incubation time distribution.

%Building on the
Without loss of generality, we %consider the Independent Cascade Model \cite{kempe2003maximizing}, and 
assume that every infected node in a cascade $c$ gets infected through one of its neighbors, and therefore the diffusion process propagates as a directed tree ${\tree}$. For a cascade $c$, each possible way in which a diffusion process can spread over the underlying network $G$ creates a tree. 
%\bm{However, our framework doesn't depend on this assumption, and a Directed Acyclic Graph (DAG) can be used instead.}
 %Therefore, all the possible diffusion trees are equally likely 
%Therefore, assuming the same prior probability of transmission over the edges of the underlying network,
For any cascade $c$, the probablity of the cascade given a diffusion tree $T$ in a network model $\mathcal{M}$ with parameter vector $\theta$ can be written as:
\begin{equation}
%f^t(c|\tree, \theta) \propto \prod_{(u,v) \in E_{\tree}}f_c^t(e_{uv}|t^c_u, t^c_v, \theta),
p(t^c|\tree, \theta, \mathcal{M}) \propto \prod_{e_{uv} \in E_{\tree}}p(e_{uv}|\theta,\mathcal{M}),
\end{equation}
%Therefore, having a conditional independence between cascades given the network $G$, the joint likelihood of a set $C$ of cascades in the network $G$ can be calculated as:
where $E_T$ is the set of edges in tree $T$.  Note that for a given cascade, all diffusion trees have the same $|E_T|=|V_T|-1$ number of edges, where $|V_T|$ is the number of infected nodes in the cascase. %$p(e_{uv}|\theta,\mathcal{M})$ is the probability of edge $e_{uv}$ in the network model (\ref{eq:mdnd}). 

Initially, without any prior knowledge about the structure of the underlying network, we define $\Delta^c_{uv}=t^c_v-t^c_u$ for all $t^c_u < t^c_v < \infty$, and initialize $p(e_{uv}|\theta,\mathcal{M}) \propto \sum_{c \in C} \Delta^c_{uv}$ for all the potential edges between infected nodes in different cascades. For the rest of the edges $e_{uv}$, for which $t^c_u = \infty$ or $t^c_v = \infty$, in all cascades,  we initialize $p(e_{uv}|\theta,\mathcal{M})=0$.

To build our list of observations, we only consider the most probable directed tree $\hat{T}_c$ supported by every cascade $c \in C$. I.e.,
\begin{equation}
\hat{T}_c = {\arg\max}_{\tree \in \mathcal{T}_c} p(t^c|\tree, \theta, \mathcal{M}),
\end{equation}
where $\mathcal{T}_c$ is the set of all the diffusion trees supported by cascade $c$.
%Note that the set of trees $\mathcal{T}_c$  supported by cascade $c$ doesn't change over time.
%Therefore, at any time $t$, 
Our final observation list $X$ consists of all the edges in the most probable trees supported by the set of cascades $c \in C$.
\begin{equation}
%X = \{ \cup_{c\in C} e_{uv} \in E_{\hat{T}_c} \}
X = \{E_{\hat{T}_{c_1}}, \cdots, E_{\hat{T}_{c_{s}}} \}
\end{equation}

%We further assume that the edges $e_{uv} \in X$ are weighted. At any time $t$, we consider the weight $w^t_{uv} \in \mathbb{Z}$

 Note that each edge can be observed multiple times. The number of observations $n_{uv}$ correspond to $e_{uv}$ is the number of the most probable trees containing edge $e_{uv}$. I.e.,
\begin{equation}
n_{uv} = \sum_{c \in C} \mathbb{I} [e_{uv} \in \hat{T}_c]
\end{equation}
The pseudocode for collecting the list observations from diffusion cascades is shown in Algorithm \ref{alg:tree}.

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\Require Set of infection times $\{t^{c_1}, \cdots, t^{c_{s}}\}$.
		\Ensure List of observations $X$.
		\State $X \leftarrow \{\}$
		\For {$c \in C$}
			\State $T_c \leftarrow \{\}$
			\ForAll {0 < $t^c$ < $\infty$}
			%			\State $ParT(i) = {\arg \max}_j p(e_{uv}|\theta) ( 1 + e^{-(t_v^c-t_u^c)})$
			%%% \State $u = \{  {\arg \max}_{v \in c} f^{t}_{c}(e_{uv}|t^c_u, t^c_v, \theta)  \}$
			\State $u = \{  {\arg \max}_{i: t^c_i < t^c_v < \infty} p(e_{iv}|\theta, \mathcal{M})  \}$
			\State $T_c \leftarrow T_c \cup \{e_{uv}$\}
			\EndFor
			\State $X \leftarrow \{X, T^c\}$
		\EndFor
		%\State \Return{ $X$}
	\end{algorithmic}
	\caption{\textsc{Collect\_Observations}}
	\label{alg:tree}
\end{algorithm}



\subsection{Updating Latent Model Variables}
To update the posterior distribution of the latent model variables conditioned on the observations, we need to resort to approximate inference. %There are two major paradigms in approximate inference: Variational and Monte Carlo inference. 
Here, we use a collapsed Gibbs sampler \cite{teh2005sharing} --a Markov chain Monte Carlo (MCMC) algorithm-- to approximate the posterior distribution of the latent variable in our hierarchical mixture model.

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\Require Parameter vector $c_{1:M}, p_{1:M}, \beta_{1:N}$, Set of infection times $\{t^{c_1}, \cdots, t^{c_{s}}\}$.
		\Ensure Updated parameter vector $c_{1:M}, p_{1:M}, \beta_{1:N}$
		%\State Initialize $c_{uv}$ randomly.
		%		\For {$t = 1, 2, \cdots t_{\max}$}
		\For {$i = 1, 2, \cdots $ until convergence}
		\State $X \leftarrow$ Collect\_Observations($\{t^{c_1}, \cdots, t^{c_{s}}\}$)
		\For {$j = 1, 2, \cdots $ until convergence}
		\State Select $e_{uv}$ randomly from $X$
		\State Sample $c$ from the conditional distribution $p(c_{uv}=k|u,v,c_{1:M}^{\neg e_{uv}} , {\beta}_{1:N} )$ \Comment{Eq. \ref{eq:pc}}
		\State Sample $e$ from the conditional distribution $p(e_{uv} = e_{ij}| {c_{1:M}}, e_{1:M}^{\neg e_{uv}}, {\beta_{1:N}})$  \Comment{Eq. \ref{eq:pe}}
		\State Sample $\rho$ from the conditional distribution $p(\rho^{(k)}_{u.} = \rho | c_{1:M}, \rho^{(k) \neg e_{uv}}_{u.}, \beta_{1:N})$ \Comment{Eq. \ref{eq:pr}}
		\State Sample $(\beta_1, \cdots, \beta_{|V|}, \beta_u) \sim \text{Dir}(\rho_{1}^{(.)}, \cdots,  \rho_{|V|}^{(.)}, \gamma)$ \Comment{Eq. \ref{eq:pb}}
		\EndFor
		\EndFor
		%\State \Return{ $\mathcal{M}(c_{1:M}, p_{1:M}, \beta_{1:N})$}
		%		\EndFor
	\end{algorithmic}
	\caption{\textsc{Update\_Network\_Model}}
	\label{alg:infer}
\end{algorithm}

\paragraph{Sampling $\pmb{c}$.}
Following \cite{williamson2016nonparametric}, we model the posterior probability for an edge $e_{uv}$ to belong to cluster $k$ as a function of the importance of the cluster in the network, and the importance of $u$ as a source and $v$ as a destination in cluster $k$, as well as the importance of $u,v$ in the network. To this end, we measure the importance of a cluster by the total number of its edges, i.e., $\eta_k = \sum_{u,v \in V} [\mathbb{I}_{c_{uv}}=k]$. Similarly, the importance of $u$ as a source, and the importance of $v$ as a destication %the source and destination of $e_{uv}$ 
in cluster $k$ is measured by the number of outlinks of $u$ associated with cluster $k$, i.e. $l_{u.}^{(k)}$, as well as inlinks of $v$ associated with cluster $k$, i.e. $l_{.v}^{(k)}$.  %$\{|e_{uv}| \xmid c_{uv}=k|\}$
Finally, the importance of a node $i$ in the network is determined by the probability mass of the edges associated with it, i.e. $\beta_i = \sum {h_{i.}} + \sum {h_{.i}}$.
The distribution over the cluster assignment $c_{uv}$ of an edge $e_{uv}$, given the end nodes $u, v$, the cluster assignments for all other edges, and $\beta$ is given by:
\begin{equation}\label{eq:pc}
p(c_{uv}=k|u,v,c_{1:M}^{\neg e_{uv}} , {\beta}_{1:N} ) \propto 
\begin{cases}
	\eta^{\neg e_{uv}}_k (l^{(k) \neg e_{uv}}_{u.} + \tau \beta_u) (l^{(k) \neg e_{uv}}_{.,v} + \tau \beta_v ) & \text{if} ~  \eta^{\neg e_{uv}}_k > 0\\
	\alpha \tau^2 \beta_u \beta_v & \text{if} ~  \eta^{\neg e_{uv}}_k = 0
\end{cases}
\end{equation}
where $\neg e_{uv}$ is used to exclude the current observation. As discussed in section \ref{sec:dynamic}, $\alpha$, $\tau$, and $\gamma$ controls the number of clusters, cluster overlaps, and the number of nodes in the network. Moreover, $N, M$ are the number of nodes and edges in the network.




\paragraph{Sampling $\pmb{e}$.}
Due to the edge-exchangeability, we can treat $e_{uv}$ as the last variable being sampled. %, and compute the conditional distribution of $e_{uv}$ given the rest of the variables. 
The conditional posterior for $e_{uv}$ given the rest of the variables can be calculated as:
\begin{equation}\label{eq:pe}
\begin{aligned}
p(e_{uv} = e_{ij}| {c_{1:M}}, & e_{1:M}^{\neg e_{uv}}, {\beta_{1:N}}) =\\
&\begin{cases}
	 \sum_{k=1}^{K+} \frac{\eta_k}{M + \alpha} \frac{l^{(k) \neg e_{uv}}_{u.} + \tau \beta_u}{\eta_k + \tau} \frac{l^{(k) \neg e_{uv}}_{.,v} + \tau \beta_v}{\eta_k + \tau} + \frac{\alpha}{M+\alpha} \beta_u \beta_v  & \text{if} ~ i,j \in V\\
	 \sum_{k=1}^{K+}  \frac{\eta_k}{M + \alpha} \frac{l^{(k) \neg e_{uv}}_{u.} + \tau \beta_u}{\eta_k + \tau} \beta_n  + \frac{\alpha}{M+\alpha} \beta_u \beta_n  & \text{if} ~ i\in V, j \notin V\\
	 \sum_{k=1}^{K+}  \frac{\eta_k}{M + \alpha} \frac{l^{(k) \neg e_{uv}}_{.,v} + \tau \beta_u}{\eta_k + \tau}  \beta_n + \frac{\alpha}{M+\alpha} \beta_n \beta_v  & \text{if} ~ i \notin V, j \in V\\
	 \beta_n^2   & \text{if} ~ i,j \notin V
\end{cases}\\
\end{aligned}
\end{equation}
where $\beta_n = \sum_{i=N+1}^\infty h_i$ is the probability mass for all the edges that may appear in the network in the future. We observe that an edge may appear between existing nodes in the network, or because one or two nodes has appeared in the network. Note that the predictive distribution for a new link to appear in the network can be calculated similarly using Eq. \ref{eq:pe}.

\paragraph{Sampling \pmb{$\rho$.}}
The probability mass on the outlinks and inlinks of a node $i$ associated with cluster $k$ are modeled by variables $\rho^{(k)}_{i.}$ and $\rho^{(k)}_{.i}$.
The posterior distribution of $\rho^{(k)}_{u.}$ (similarly $\rho^{(k)}_{.v}$), can be calculated using:
\begin{equation}\label{eq:pr}
	p(\rho^{(k)}_{u.} = \rho | c_{1:M}, \rho^{(k) \neg e_{uv}}_{u.}, \beta_{1:N}) = \frac{\Gamma(\tau \beta_u)}{\Gamma(\tau \beta_u + l_{u.}^{(k)})} s(l_{u.}^{(k)}, \rho)(\tau \beta_u)^{\rho},
\end{equation}
where $s(l_{u.}^{(k)}, \rho)$ are unsigned Stirling numbers of the first kind. I.e., $s(0, 0) = s(1, 1) = 1, s(n, 0) = 0$ for $n > 0$ and $s(n,m) = 0$ for $m > n$. Other entries can be computed as $s(n + 1,m) = s(n,m - 1) + ns(n,m)$.
However, for large $l_{u.}^{(k)}$, it is often more efficient to sample $\rho_{k,i}$ by simulating the table assignments of the Chinese restaurant according to Eq. \ref{eq:pe} \cite{fox2007sticky}.

\paragraph{Sampling $\pmb{\beta}$.}
%$\beta_i = \sum_{i=|V^t|+1}^\infty h_i$
Finally, the distribution of edges of the nodes in the network is modeled by a Dirichlet distribution, i.e., 
\begin{equation}\label{eq:pb}
(\beta_1, \cdots, \beta_{N}, \beta_n) \sim \text{Dir}(\rho_{1}^{(.)}, \cdots,  \rho_{N}^{(.)}, \gamma),
\end{equation}
where $\rho^{(.)}_i = \sum_k\rho^{(k)}_{i.}+\rho^{(k)}_{.i}$.

The pseudocode for inferring the latent network variables from diffusion data is given in Algorithm \ref{alg:infer}.




\subsection{On-line Dynamic Network Inference}

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\Require Set of infection times $\{t^{c_1}, \cdots, t^{c_{s}}\}$, interval length $w$.
		\Ensure Updated network model $\mathcal{M}^t$ at any time $t=iw$.
		\State $t=w$, initialize $\mathcal{M}^0$ randomly. 
		\While{$t < $ last infection time}
		%\State $Y^t \leftarrow \emptyset$
		\ForAll {$c \in C$}
			\State $t^{cw} \leftarrow t^c_u \in [t-w, t)$
			\State $Y^t \leftarrow \{Y^t, t^{cw}\}$
		\EndFor
		\State $\mathcal{M}^{t} \leftarrow $ Update\_Network\_Model($\mathcal{M}^{t-w}, Y^t$) 
		\State $t = t + w$.
		%\State \Return{ $\mathcal{M}^{t}$}
		\EndWhile
	\end{algorithmic}
	\caption{\textsc{Dynamic\_Network\_Inference (\alg)}}
	\label{alg:dyference}
\end{algorithm}

In order to capture the dynamics of the underlying network and keep the  model updated over time, we consider time intervals of length $w$. For the $i$-th interval, we only consider the infection times $t^c \in [(i-1)w, iw)$ for all $c \in C$, and update the model conditioned on the observations in the current time interval. 
There is a trade-off between the speed of tracking changes in the underlying network structure, and the accuracy of our algorithm. For smaller intervals, we incorporate new observations more rapidly, and therefore we are able to track changes faster. On the other hand, for larger intervals we have a higher number of observations from each cascade. Hence, the most probable tree supported by each cascade is larger, and can provide more information about the network structure.

Note that we don't infer a new model for the network based on infection times in each time interval. Instead, we use new observations to \textit{update} the latent variables from the previous time interval. Updating the model with observations in the current interval results in a higher probability for the observed edges, and a lower probability for the edges that have not been observed and the size of %probability mass on 
their neighborhood --in terms of the degree of the two end nodes-- hasn't been increased.
Therefore, we don't need to consider an aging factor to take into account the older cascades. The pseudocode of our dynamic inference method is given in Algorithm \ref{alg:dyference}.




==> sections/4_experiment_copy.tex <==
% !TEX root=../nips_2018.tex
\section{Experiments}
\label{sec:Experiments}
In this section, we address the following questions: 1) How good is the predictive performance of \alg in static and dynamic networks compared to the existing network inference algorithms? 2) How does predictive performance of \alg change with the number of cascades? 3) How does running time of \alg compared to the baselines?
%We evaluate the performance of \alg on three benchmark tasks: (i) impact of number of cascades using the static synthetic dataset, (ii) clarifying how our method allows adoption to the changes of the underlying time-varying network, using both synthetic and real-world datasets, (iii) analyzing the time complexity over real-world datasets and (iv) predicting most influential users using MemeTracker dataset.

%We show that \alg outperforms the baselines in different network topologies and we validate our results and demonstrate the effectiveness of our method in both static and dynamic scenarios.
%, where the existing on-line algorithm (InfoPath) is incapable of providing reasonable performance for the network inference problem.
%Moreover, we use the influence maximization method[?] over the inferred networks to compare how accurate our algorithm can detect the most influential users comparing to the baseline.
\textbf{Baselines.}  We compare the performance of \alg to \textsc{NetInf}~\cite{gomez2012inferring}, \textsc{NetRate}~\cite{rodriguez2011uncovering}, \textsc{TopoLstm}~\cite{bourigault2016representation} and \textsc{InfoPath}~\cite{gomez2013structure}. \textsc{InfoPath} is the only method able to infer dynamic networks, hence we can only compare the performance of \alg on dynamic networks with \textsc{InfoPath}.

%\textbf{Baselines.}  We compare the performance of \alg with \textsc{NetInf}~\cite{gomez2012inferring}, \textsc{NetRate}~\cite{rodriguez2011uncovering}, %\textsc{TopoLstm}~\cite{bourigault2016representation} and \textsc{InfoPath}~\cite{gomez2013structure} for predicting the edges of the underlying diffusion network. \textsc{NetInf}, \textsc{NetRate} and %\textsc{TopoLstm} are only able to infer edges of static networks, therefore we only compare our results on dynamic networks with \textsc{InfoPath}.

\textbf{Evaluation Metrics.} For performance comparison, we use Precision, Recall and F1 measure of inferred edges as well as the Mean Squared Error (MSE) in the edge transmission rate. Precision
is the fraction of edges in the inferred network present in the true network, Recall is the fraction of edges of the true network present in the inferred network, and F1 measure is 2$\times$(precision$\times$recall)/(precision+recall). MSE is the mean-squared-error measure between predicted and true probabilities. We also use Hits@$k$ that is the rate of the top-$k$ ranked nodes containing the next active node, and MAP@$k$ that is the classical mean average precision measure.

%We evaluate performance of our method by computing three different measures: Accuracy, Precision and Recall. Precision is the fraction of edges in the inferred network $\hat{G}^t$present in the true network $G^{\ast t}$. Recall is the fraction of edges of the true network present in the inferred network. Accuracy is $1- \frac{\sum_{u,v} |\mathbb{I}(p_{uv}^{\ast t})-\mathbb{I}(\hat{p}_{uv}^t)|} {\sum_{u,v}\mathbb{I}(p_{uv}^{\ast t})+\mathbb{I}(\hat{p}_{uv}^t)}$, where $\mathbb{I}(p_{uv}^t)=1$ if $p_{uv}^t>0$ and $\mathbb{I}(p_{uv}^t)=0$ otherwise. Moreover, we use two ranking metrics (varying $k$ in $\{10,50,100\}$); (1) \textit{Hits@$k$}: is the rate of top-$k$ ranked predicted edges, and (2) \textit{MAP@$k$}: is the classical Mean Average Precision measure.

\textbf{Experiments on synthetic data.}
%To evaluate the performance of \alg on static networks, 
We generated synthetic networks consist of 1024 nodes and about 2500 edges using Kronecker graph model~\cite{Leskovec:2007:SMR:1273496.1273559}: core-periphery network (CP)[0.9,0.5;0.5,0.3], hierarchical community network (HC)[0.9,0.1;0.1,0.9], %random network (RD)[0.5,0.5;0.5,0.5], 
and the Forest Fire model~\cite{leskovec2005densification}: with forward and backward burning probability 0.2 and 0.17. 
%
For dynamic networks, we assign a pattern to each edge uniformly at random from a set of five edge evolution patterns: Slab, Square, Chainsaw, Hump and Constant and the transmission rates are generated for each edge according to its chosen evolution pattern for 100 time steps. We then generate 500 information cascades per time step on the network  with the random initiator node for each cascade \cite{gomez2011uncovering} .

%Figure~\ref{fig:syn_num_casc} shows accuracy, precision and recall of the \alg method compared to the static baselines for varying number of cascades in the Kronecker and the Forest Fire networks. It can be seen that \alg obtained a very good result for accurately inferring the diffusion network for all types of network.
%As illustrated in the Figure~\ref{fig:dy_syn}, \alg almost always outperforms \textsc{InfoPath} in different time intervals. We note that the performance of our method is stable over time.






\textbf{Experiments on Real data.}
We applied \alg to two real wold datasets, %Memes and Twitter. 
1)  Twitter~\cite{DBLP:journals/corr/HodasL13a} contains the diffusion of URLs on Twitter during 2010 and the follower graph of users. The network consists of 137,093 nodes and 3,589,811 edges with 569 cascades of length of 5.7 in average and 2) Memes~\cite{Leskovec:2009:MDN:1557019.1557077} contains the diffusion of memes from March 2011 to February 2012 over online news websites; The real diffusion network is constructed by the temporal dynamics of hyperlinks created between news sites. The network consists of 5,000 nodes and 313,669 edges with 54,847 cascades of length of 17 in average. %Table \ref{table:topic} summarizes the number of sites and meme cascades for several topics and real world events. 

\begin{figure*}[t]
	\vspace{-.3cm}
	\centering  
	%[width=.35\textwidth,height=.23\textwidth]
	\subfloat[CP - Exp\label{subfig:cpexp}]{
		\includegraphics[width=.25\textwidth,trim= 0mm 0 10mm 0]{figs/dynamic/KR_CP_exp_plot_Accuracy_Time.pdf}
		\includegraphics[width=.25\textwidth,trim= 7mm 0 4mm 0]{figs/dynamic/KR_CP_exp_plot_Precision_Recall.pdf}}
	\subfloat[HC - Ray\label{subfig:hcray}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/dynamic/KR_HC_ray_plot_Accuracy_Time.pdf}
		\includegraphics[width=.25\textwidth,trim= 7mm 0 4mm 0]{figs/dynamic/KR_HC_ray_plot_Precision_Recall.pdf}}\\
	%	\caption{Precision-Recall and Accuracy of \alg for inferring dynamic diffusion networks compared to \textsc{InfoPath} in each time interval. (a,b) CP-Kronecker network with exponential edge transmission model, (c,d) HC-Kronecker network with rayleigh edge transmission model.}
	%	\label{fig:dy_syn}
	%\end{figure*}
	%\begin{figure*}[!htb]
	\vspace{-.4cm}
	%  \centering  
	%[width=.35\textwidth,height=.23\textwidth]
	\subfloat[HC - Ray\label{subfig:hc_ray}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/static/num_cascades/plot_accuracy_num-Cascades_KR_HC_.pdf}}%\hspace{5mm}
	\subfloat[CP - Exp\label{subfig:cp_exp}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/static/num_cascades/plot_accuracy_num-Cascades_KR_CP_.pdf}}
	\subfloat[FF - Pwl\label{subfig:ff_pwl}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/static/num_cascades/plot_accuracy_num-Cascades_FF_.pdf}
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/meme/MemeDatasets_Running_time.pdf}}
	%\caption{Accuracy of the \alg compared to static baselines over number of cascades. (a) HC-Kronecker network with Rayleigh transmission model and, (b) CP-Kronecker network with Exponential transmission model.}
	%\label{fig:syn_num_casc}
	%\end{figure*}
	%\begin{figure*}[!htb]
	\vspace{-.3cm}
	%	\begin{minipage}{1\linewidth}
	%		\centering  
	%[width=.35\textwidth,height=.23\textwidth]
	\subfloat[Occupy\label{subfig:occupy}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/meme/occupy_plot_Accuracy_Time.pdf}}
	%			\includegraphics[width=.25\textwidth]{figs/meme/occupy_plot_Precision_Recall.pdf}}%\hspace{5mm}
	\subfloat[Linkedin\label{subfig:linkedin}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/meme/linkedin_plot_Accuracy_Time.pdf}}
	%			\includegraphics[width=.25\textwidth]{figs/meme/linkedin_plot_Precision_Recall.pdf}}
	%	\end{minipage}
	%	\begin{minipage}{1\linewidth}
	\subfloat[NBA\label{subfig:nba}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/meme/nba_plot_Accuracy_Time.pdf}}
	%			\includegraphics[width=.25\textwidth]{figs/meme/nba_plot_Precision_Recall.pdf}}
	\subfloat[News of The World)\label{subfig:nba}]{
		\includegraphics[width=.25\textwidth,trim=0mm 0 10mm 0]{figs/meme/newsoftheworld_plot_Accuracy_Time.pdf}}
	%			\includegraphics[width=.25\textwidth]{figs/meme/newsoftheworld_plot_Precision_Recall.pdf}}
	%	\end{minipage}
	\label{fig:memes}
	\caption{Precision, Recall, and Accuracy of \alg for the time-varying hyperlink network with four different topics over time from March 2011 to July 2011.}
\end{figure*}


\begin{minipage}{\textwidth}

\begin{minipage}[b]{0.45\textwidth}
\centering
%		\small
 \begin{tabular}{||lccc||}
	 \hline
	 \small
	 Topics & $\#$sites &$\#$ hyperlinks& $\#$memes \\ \hline
	 NBA &2,087&142,738&1,543,630 \\ \hline
	 Occupy &1,875&44,911&655,183 \\ \hline
	 Linkedin &1,035&22,964&155,755 \\ \hline
	 News  &1,035&64,619&101,836 \\ \hline
 \end{tabular}
\captionof{table}{Statistics of Topics of Meme Dataset}
\end{minipage}
\hfill
\begin{minipage}[b]{0.54\textwidth}
\begin{center}
%{\includegraphics[width=.54\textwidth, trim=5mm 0mm 10mm 15mm]{figs/meme/MemeDatasets_Running_time.pdf}}
%\captionof{figure}{Running time of Memes Dataset.}
\end{center}
\end{minipage}
\end{minipage}
%%nba & 2,056&142,738&11,955,546\\ \hline
%al qaeda & 1,142&44,911&8,955,039\\ \hline
%linkedin & 1,035&22,964&9,215,167\\ \hline
%news of the world & 1,390&64,619&10,546,071\\ \hline


\begin{table}[!htb]
 \begin{center}
 \small
	\begin{tabular}{|c|ccc|ccc|}
	\toprule
	& \multicolumn{3}{|c|}{Twitter} & \multicolumn{3}{|c|}{Memes} \\ 
	\midrule
	\textit{MAP@$k$} & @10 & @50 & @100 & @10 & @50 & @100 \\ 
	\midrule
	\textsc{Infopath} &&&&&& \\ 
	\textsc{TopoLstm} &&&&&& \\ 
	\textsc{Dyference} &&&&&& \\ 
	\midrule
	\textit{Hits@$k$} & @10 & @50 & @100 & @10 & @50 & @100 \\
	\midrule
	\textsc{Infopath} &&&&&& \\ 
	\textsc{TopoLstm} &&&&&& \\ 
	\textsc{Dyference} &&&&&& \\  \hline
	\end{tabular}
 \end{center}
\caption{Results on Dyference}
\label{table:topic}
\end{table}

%\subsection{Predicting Influentials}
%
%\begin{figure}[!htb]
%	\begin{center}
%		{ 
%			\subfigure[Linkedin]{\includegraphics[trim = 3mm 0mm 3mm 0mm, clip, ,scale=0.2]{figs/meme/linkedin_plot_IM_Time.pdf}
%				\includegraphics[trim = 3mm 0mm 3mm 0mm, clip, ,scale=0.2]{figs/meme/linkedin_IM_plot_Precision_Recall.pdf}}
%			\subfigure[Occupy]{\includegraphics[trim = 3mm 0mm 3mm 0mm, clip, ,scale=0.2]{figs/meme/occupy_plot_IM_Time.pdf}
%				\includegraphics[trim = 3mm 0mm 3mm 0mm, clip, ,scale=0.2]{figs/meme/occupy_IM_plot_Precision_Recall.pdf}}
%		}
%		%\vspace{-.4cm}
%	\end{center}
%	\caption{Influential Users at the end of every 30 days.}
%	\label{fig:influentials}
%	%\vspace{-.4cm}
%\end{figure}

\begin{table}[!htb]
	\begin{center}
		\small
		\begin{tabular}{|c|c|c|}
			\hline
			Ground Truth& \alg & \textsc{InfoPath}\\ \hline \hline
			elmundo.feedsportal.com &\textbf{da.feedsportal.com}& scribd.com\\ \hline
			thestar.com.my.feedsportal.com &quizilla.teennick.com&redorbit.com \\ \hline
			article.wn.com &seattletimes.nwsource.com&theage.com.au \\ \hline
			tin247.com &\textbf{yachtchartersmagazine.com}& allafrica.com\\ \hline
			da.feedsportal.com  &news.yahoo.com&signonsandiego.com\\ \hline
			firmenpresse.de &\textbf{article.wn.com}& canadaeast.com\\ \hline
			yachtchartersmagazine.com  &\textbf{ctv.ca}&news.yahoo.com\\ \hline
			france24.com &\textbf{fair-news.de}& proceso.com.mx\\ \hline
			ctv.ca &fanfiction.net& \textbf{article.wn.com}\\ \hline
			fair-news.de &bbc.co.uk&prnewswire.com \\ \hline
		\end{tabular}
	\end{center}
	\caption{Example of Top 10 Influential websites of Meme Dataset on 30-06-2012}
	\label{table:topic}
\end{table}


%\subsection{Run time Comparision}


==> sections/6_ExperimentalEvaluation.tex <==
\section{Experiments}
\label{sec:Experiments}
In this section, we apply our algorithm to several network settings. First, we show that how our method outperforms the baseline in case of static networks. Then, we validate our results and demonstrate the effectiveness of our method in dynamic scenarios, where the existing on-line algorithm (InfoPath) is incapable of providing reasonable performance for the network inference problem. Moreover, we use the influence maximization method[?] over the inferred networks to compare how accurate our algorithm can detect the most influential users comparing to the baseline.
%In this section, we want to experimentally evaluate the performance of the NPNM model over synthetic and real-world networks using static and dynamic diffusion data, to address the following questions: (1) How does the accuracy of the model depend on the number of connections in the underlying network? 
%%(2) How does the average number of infected nodes in the cascades affect the accuracy of NPNM? 
%(2) How many times does the proposed method need to iterate over the information cascades in order to converge to a reasonable result compared to best existing results of the baselines? (3) How accurate does the inferred network adjust itself with the changes in dynamic diffusion network over time? (4) What is the effect of network topological structure on the \alg performance? 

The measure of performance for all methods is Accuracy, Precision, and Recall of the inferred network in comparison with the ground truth network. Precision is the fraction of edges in the inferred network present in the true network. Recall is the fraction of edges of the true network present in the inferred network. Accuracy is $1 - \frac{\sum_{i,j}|\mathbb{I}(\alpha_{i,j}^{*})-\mathbb{I}(\hat{\alpha_{i,j}})|}{\sum_{i,j}\mathbb{I}(\alpha_{i,j}^{*}) + \sum_{i,j}\mathbb{I}(\hat{\alpha_{i,j}})}$, where $\mathbb{I}(\alpha)=1$ if $\alpha > 0$ and $\mathbb{I}(\alpha)=0$ otherwise~\cite{gomez2011uncovering}. We show that the \alg outperforms the best existing methods in both static and dynamic settings by extensive experiments over various types of networks. 
\begin{figure}[t]
\begin{center}
{

\subfigure[HC, Exp]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip,,scale=0.275]{figs/static/syn1/Accuracy_Edges_KR_exp_HC_.pdf}}
%\subfigure[ray,HC]{\includegraphics[trim = 3mm 0mm 10mm 0mm, clip,,scale=0.275]{figs/static/syn1/Accuracy_Edges_KR_ray_HC_.pdf}}
\subfigure[FF, Exp]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_FF_exp_.pdf}}
%\subfigure[ray,FF]{\includegraphics[trim = 3mm 0mm 10mm 0mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_FF_ray_.pdf}}
\subfigure[HC, Pwl]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_KR_pwl_HC_.pdf}}
\subfigure[FF, Pwl]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_FF_pwl_.pdf}}
\subfigure[HC, Ray]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_KR_ray_HC_.pdf}}
\subfigure[FF, Ray]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_FF_ray_.pdf}}
%\subfigure[pwl,CP]{\includegraphics[trim = 3mm 0mm 10mm 0mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_KR_pwl_CP_.pdf}}
%\subfigure[pwl,RD]{\includegraphics[trim = 3mm 0mm 10mm 0mm, clip, ,scale=0.275]{figs/static/syn1/Accuracy_Edges_KR_pwl_RD_.pdf}}
}
\vspace{-.4cm}
\end{center}
\caption{Accuracy of the proposed \alg in comparison with the baseline methods for varying number of edges in the networks. (a,c,e) Hierarchical Community (HC) Kronecker network and (b,d,f) Forest Fire (FF) network both with Exponential (Exp), Power-law (Pwl), and Rayleigh (Ray) edge transmission models.}
\label{fig:syn1}
\vspace{-.4cm}
\end{figure}
%\begin{figure}[t]
%\begin{center}
%{
%\subfigure[CP, Pwl]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip,,scale=0.275]{figs/static/syn2/KR_pwl_CP_512_plot_accuracy_epochs.pdf}}
%\subfigure[RD, Exp]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip,,scale=0.275]{figs/static/syn2/KR_exp_RD_512_plot_accuracy_epochs.pdf}}
%\subfigure[HC, Ray]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/static/syn2/KR_ray_HC_512_plot_accuracy_epochs.pdf}}
%\subfigure[FF, Pwl]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/static/syn2/FF_pwl_512_plot_accuracy_epochs.pdf}}
%}
%\vspace{-.4cm}
%\end{center}
%\caption{Accuracy of \alg and the baselines over the number of iterations (epochs) that each method needs. (a) Core-Periphery network (CP) with power-law edge transmission model, (b) Random (RD) network with exponential edge transmission model, (c) Hierarchical Community (HC) Kronecker network with rayleigh edge transmission model, and (d) Forest Fire (FF) network with power-law edge transmission model.}
%\label{fig:syn2}
%\vspace{-.4cm}
%\end{figure}
\begin{figure}[t]
\begin{center}
{ %figs/dynamic/syn1/KR_exp_CP_0_1.0_plot_Precision_Recall.pdf
\subfigure[CP, Exp]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip,,scale=0.275]{figs/dynamic/syn1/KR_exp_CP_0_1_plot_Precision_Recall.pdf}}
\subfigure[HC, Ray]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip,,scale=0.275]{figs/dynamic/syn1/KR_ray_HC_0_1_plot_Precision_Recall.pdf}}
\subfigure[CP, Exp]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/dynamic/syn1/KR_exp_CP_0_1_plot_Accuracy_Time.pdf}}
\subfigure[HC, Ray]{\includegraphics[trim = 5mm 0mm 10mm 15mm, clip, ,scale=0.275]{figs/dynamic/syn1/KR_ray_HC_0_1_plot_Accuracy_Time.pdf}}
}
\vspace{-.4cm}
\end{center}
\caption{Precision-Recall and Accuracy of \alg in inferring dynamic diffusion networks compared to \textsc{InfoPath} with 500 cascades in each time slot. (a,c) Core-Periphery (CP) Kronecker network with exponential edge transmission model, (b,d) Hierarchical Community (HC) Kronecker network with rayleigh edge transmission model.}
\label{fig:dy-syn1}
\vspace{-.4cm}
\end{figure}  
\subsection{Baselines}
For benchmarking our model, we use three well-known methods of \textsc{NetInf}~\cite{gomez2010inferring}, \textsc{NetRate}~\cite{rodriguez2011uncovering} and \textsc{InfoPath}~\cite{gomez2013structure} as baselines. \textsc{NetInf} is a greedy algorithm which is probably the best network inference using information cascades. It infers a top-$k$-edge set by maximizing a likelihood function. \textsc{NetRate} improves the likelihood function of \textsc{NetInf} by inferring the diffusion network as well as the edge transmission rates. The transmission rate indicates how likely a diffusion edge exists between a node pair. \textsc{InfoPath} is an online algorithm for the time-varying network inference. These methods are all parameterized by the type of transmission rates over edges of the network. However, only the latter method considers the dynamicity of the underlying network and the edge transmission rates over time. We evaluate the performance of the NPNM compared to all baselines over static networks, and we set the running mode of \textsc{InfoPath} as Single Point (-rm:3). Moreover, we evaluate the performance of our method on inferring dynamic diffusion networks compared to \textsc{InfoPath} with running mode Time Step (-rm:0). We used the publicly available source code provided by the authors of these methods. \textsc{NetInf} and \textsc{InfoPath} were implemented by C++, and \textsc{NetRate} was implemented by Matlab. 
\subsection{Experiments on Synthetic Networks}
\textbf{Network Generation.} For \textbf{static} network inference, we generate two types of synthetic networks using Kronecker graph model~\cite{Leskovec:2007:SMR:1273496.1273559} and the Forest Fire model~\cite{leskovec2005densification}, both with 512 nodes and 1024 edges. These models are widely used for analysing real-world directed social networks. We show that the proposed method can perform well on different types of network models. For the Kronecker graph model we adopt three different networks with different parameters same as ~\cite{gomez2011uncovering}: core-periphery network (CP)[0.9,0.5;0.5,0.3], hierarchical community network (HC) [0.9,0.1;0.1,0.9], and random network (RD) [0.5,0.5;0.5,0.5]. For the Forest Fire model (FF), we generate a directed network with forward burning probability 0.2 and backward burning probability 0.17. For generating synthetic networks in \textbf{dynamic} settings, we also need to specify the time-varying transmission rates of edges over time. We use the settings in~\cite{GomezRodriguezLS2013b} which assigns a pattern to each edge uniformly at random from a set of five edge evolution patterns: Slab, Square, Chainsaw, Hump and Constant. Then, the transmission rate values are generated for each edge according to its chosen evolution pattern for 100 time slots.

\textbf{Cascade Generation.} To simulate several cascades over synthetic networks in static settings, we use the generative approach of~\cite{gomez2011uncovering}. In this method one can generate a cascade set based on three transmission models (i.e. Exponential, Power-law, or Rayleigh). There are two parameters in the cascade setting. $\alpha$ is the transmission rate of a transmission model, and $\beta$ controls the cascade length. We use the same setting as~\cite{gomez2011uncovering} and set $\alpha=[0.01,2]$ and $\beta$=0.4 (for core-periphery $\beta$=0.1). We pick the starting nodes uniformly at random and generate 500 cascades for each network. In the experiment in which we want to show the effect of number of edges on the accuracy of the model, we generate as many cascades as needed to cover $95\%$ of the edges in the underlying network. In dynamic settings, we generate 500 cascades per time slot and considering one type of edge transmission rate for each network that we are generating the cascades over.

\textbf{Results.} Figure~\ref{fig:syn1} shows the accuracy of the NPNM method compared to the baselines for varying number of edges in the Kronecker and the Forest Fire networks. In this case, we exponentially increase the node size from $|V|=2^5$ to $|V|=2^{10}$ in order to accordingly change the number of edges in the underlying network. For each number of edges, we generate as many cascades as they cover 95\% of network edges. This setting ensures that \textsc{NetInf} performs its best. As depicted in the figure, the NPNM method yields a very good results for accurately inferring the diffusion network for all types of network which emphasizes on its non-parametric nature. \textsc{NetInf} performs better than the other competing methods, while \textsc{InfoPath} is the worst one in terms of accuracy of estimating the static diffusion network. \textsc{NetRate} works well for the networks with the power-law transmission model, however its accuracy degrades in the networks with the exponential transmission model. As we expected, \textsc{NetInf} as the best greedy algorithm performs well, but the interesting point is that the NPNM as a non-parametric model can infer the diffusion network with similar accuracy. 

%After evaluating the accuracy of the proposed method, another important measure that needs to be taken into consideration is the number of iterations (epochs) that a method needs to accurately infer the diffusion network. Since, our method and the baselines were implemented in different programming languages (\textit{i.e.} C++, Matlab, Python), comparing their running time is not fair enough, instead we chose the number of required epochs. Figure~\ref{fig:syn2} shows the effect of number of epochs on the accuracy of the methods for static network inference task. The results depicts that the NPNM method performs better than the baselines in which it can accurately infer the underlying network structure with a few number of iterations. It is worth noting that our non-parametric model can reach high accuracy in different types of network models with various transmission rates. The setting of \textsc{InfoPath} for static networks is single time step which only needs one iteration to return one result. Although \textsc{InfoPath} is much faster than the other baselines, it penalizes the accuracy of inferring a static network. It is clear that with the same number of information cascades, \textsc{NetInf} and \textsc{NetRate} require many iterations to estimate the network structure with the same accuracy as our NPNM method. 

Now, we evaluate the performance of the proposed method against dynamic diffusion data. Since \textsc{InfoPath} is the only method among the baselines that can estimate dynamic networks, we compare the NPNM with this method in terms of Precision-Recall and accuracy in Figure~\ref{fig:dy-syn1}. As illustrated in the figure, the proposed method almost always performs better than \textsc{InfoPath} in different time slots. In Figure~\ref{fig:dy-syn1}(a,b), the NPNM as a non-parametric network model has almost constant Precision-Recall for different time slots and also for different network models with different transmission rates. However, the Precision-Recall of \textsc{InfoPath} in HC Kronecker network with Rayleigh transmission model is higher than that of CP Kronecker network with Exponential transmission model. This observation is similar for Figure~\ref{fig:dy-syn1}(c,d) in which the accuracy of NPNM is around 0.7 for both network models with different transmission rates, however the accuracy of \textsc{InfoPath} in HC network is higher than that of CP network. Moreover, the accuracy of \textsc{InfoPath} has a decreasing trend over time. 

One can conclude that the NPNM method is a better and more stable approach for inferring static/dynamic diffusion networks in comparison with the best existing baselines.
%Finally, we evaluate the effects of the approximate ? in figure .. As evident from the figure the gains from the .. and it seems that .. approximately does not strongly affect the results
%
%To demonstrate the scalability of our method and obtain a better qualitative understanding of the resulting marginals, we ran on a real world
%image segmentation task.We use the same setting, data and models as [1], as implemented in .. Because
%libDAI
%was too slow, we wrote our own TRWBP implementation.
%Figure 6 shows the results for two specific images ?. The example in the first row is particularly difficult for pairwise models, but the rich higher-order model has no problem capturing the details even in the challenging shaded regions of the image. The second row shows results for two different model parameters. The second model uses a function ? that is closer to being linear, while the first one is more curved (see the appendix for details). We observe that ? requires lower temperature parameters (i.e. relatively larger functions ?/) , and that the bottleneck of the complete inference procedure is running the ? updates. In other words,the added complexity from our method is minimal and the runtime is dominated by the message passing updates of TRWBP. Hence, any algorithms that speed up TRWBP (e.g., by parallelization or better message scheduling) will result in a direct improvement on the proposed inference procedure.

\subsection{Experiments on Real Networks}
We employ the real data sets of memeTracker~\cite{Leskovec:2009:MDN:1557019.1557077}. memeTracker is a tool to track quotes and phrases across the mass media and personal blogs over time. The data set consists of more than 300 article records in 3.3 million websites over a period of one year, from March 2011 to February 2012. The propagation of the short textual phrases called \textit{memes} through the Web is traced in this data set. Each meme can be considered as a separate information cascade which contains the timestamp and the URLs of cited meme. 
%By using these citations, one can trace the cascade of a particular meme. 
A cascade starts on a meme which is first published on the Web. The following articles in the cascade cite the first article directly or indirectly. 
%The time stamps of all articles are measured by hours. 
The real diffusion network is constructed by the temporal dynamics of hyperlinks created between news sites. By discretizing the time in days and generating a network per day, an edge $e_{uv}$ is added to the network if a document on site $u$ cited a document on site $v$ within the last day. 

In our experiments, we first try to infer the time-varying network per day from the hyperlinks cascades. Second, we evaluate the accuracy of our model comparing to the real diffusion network in each day and then, we compare the results with \textsc{InfoPath}. We focus on the memes of three topics as described in Table~\ref{table:topic}.
\begin{table}
\vspace{-.4cm}
\begin{center}
\small
\begin{tabular}{||lcc||}
\hline
%Topic (Network) & $\#$sites(nodes) & $\#$hyperlink s(edges) & $\#$cascades  \\ [.5ex] \hline \hline 
%%nba & 2,056&142,738&11,955,546\\ \hline
%al qaeda & 1,142&44,911&8,955,039\\ \hline
%linkedin & 1,035&22,964&9,215,167\\ \hline
%news of the world & 1,390&64,619&10,546,071\\ \hline
Topics or news event & $\#$sites (nodes) & $\#$memes (cascades)\\ \hline
Amy Winehouse &1,207&109,650 \\ \hline
Fukushima &1,666&383,745 \\ \hline
Gaddafi &1,358& 440,646\\ \hline
Kate Middleton &1,427&191,777 \\ \hline
NBA &2,087&1,543,630 \\ \hline
Alqaeda &1,142& 259,811 \\ \hline
Occupy &1,875&655,183 \\ \hline
Strauss-Kahn &1,263&204,238 \\ \hline
Linkedin &1,035&155,755 \\ \hline
News of the World &1,035&101,836 \\ \hline
\end{tabular}
\end{center}
\caption{Statistics of the Datasets}
\label{table:topic}
\vspace{-.6cm}
\end{table}
\begin{figure*}
\begin{center}
{ %figs/dynamic/syn1/KR_exp_CP_0_1.0_plot_Precision_Recall.pdf
\subfigure[al quaeda]{\includegraphics[trim = 6mm 0mm 16mm 15mm, clip,,scale=0.2]{figs/meme/alqaeda_plot_Accuracy_Time.pdf}\includegraphics[trim = 6mm 0mm 16mm 15mm, clip,,scale=0.2]{figs/meme/alqaeda_plot_Precision_Recall.pdf}}
\subfigure[news of the world]{\includegraphics[trim = 6mm 0mm 16mm 15mm, clip,,scale=0.2]{figs/meme/newsoftheworld_plot_Accuracy_Time.pdf}\includegraphics[trim = 6mm 0mm 16mm 15mm, clip,,scale=0.2]{figs/meme/newsoftheworld_plot_Precision_Recall.pdf}}
\subfigure[linkedin]{\includegraphics[trim = 6mm 0mm 16mm 15mm, clip,,scale=0.2]{figs/meme/linkedin_plot_Accuracy_Time.pdf}\includegraphics[trim = 6mm 0mm 16mm 15mm, clip,,scale=0.2 ]{figs/meme/linkedin_plot_Precision_Recall.pdf}}
}
\vspace{-.4cm}
\end{center}
\caption{Precision, Recall, and Accuracy of \alg for the time-varying hyperlink network with three different topics over time for April 2011.}
\label{fig:real}
\vspace{-.4cm}
\end{figure*}


\textbf{Results.} Figure~\ref{fig:real} shows the Accuracy, Precision and Recall over time for the dynamic network for April 2011. We set the transmission model of the edges to exponential in sake of \textsc{InfoPath} setting. We observe daily periodicity and the overall encouraging performance of around 0.4 for all three performance metrics. The results show that NPNM is more accurate than \textsc{InfoPath}. Moreover, our model performs similar in all these topics because of its non-parametric nature. Furthermore, \textsc{InfoPath} has higher Precision but a very low recall. Nevertheless, our method has almost similar Precision and Recall. Overall, one can find that NPNM has a better performance in comparison with \textsc{InfoPath} to infer the real diffusion network. 
%i.e. Exponential Model ($e^{-\alpha(t_v-t_u)}$), Power-law Model ($\frac{\alpha}{\delta}(\frac{t_v-t_u}{\delta})^{(-1-\alpha)}$) and Rayleigh Model ($\alpha(t_v-t_u)e^{-0.5\alpha(t_v-t_u)^2}$) with transmission rate $\alpha$ for edge $(u,v)$.Emron, [11.02.18 00:29]


